On contact modulo p L-space covers

The purpose of this article is to extend certain results of Roso (2023) which concerned equivariant contact structures on minimal L-spaces to the more general setting of mod p L-spaces. This is achieved by considering the Serre spectral sequence of the Borel Floer cohomology as showcased in Baraglia & Hekmati (2021). Along the way, the author introduces two new numerical invariants of equivariant contact structures which emerge from the structure of the Borel Floer cohomology as a module over the group cohomology.

==> Makefile <==
.POSIX:
.SUFFIXES:

SRC = main abs article notation maths bib intro inv \
      serre tor knot lift

OBJ = main.log main.aux main.ps main.pdf main.dvi

all: main.pdf

main.pdf: main.ps
	gs -dBATCH -dNOPAUSE -sDEVICE=pdfwrite -sOutputFile=$@ $<
main.ps: main.dvi
	dvips $<
main.dvi: $(SRC:=.tex)
	tex -interaction nonstopmode \
		-halt-on-error \
		-file-line-error \
		main.tex
	rm -fv main.log

clean:
	rm -fv $(OBJ) 

